Stabilizing Open-Set Test-Time Adaptation via Primary-Auxiliary Filtering and Knowledge-Integrated Prediction

Deep neural networks demonstrate strong performance under aligned training-test distributions. However, real-world test data often exhibit domain shifts. Test-Time Adaptation (TTA) addresses this challenge by adapting the model to test data during inference. While most TTA studies assume that the training and test data share the same class set (closed-set TTA), real-world scenarios often involve open-set data (open-set TTA), which can degrade closed-set accuracy. A recent study showed that identifying open-set data during adaptation and maximizing its entropy is an effective solution. However, the previous method relies on the source model for filtering, resulting in suboptimal filtering accuracy on domain-shifted test data. In contrast, we found that the adapting model, which learns domain knowledge from noisy test streams, tends to be unstable and leads to error accumulation when used for filtering. To address this problem, we propose Primary-Auxiliary Filtering (PAF), which employs an auxiliary filter to validate data filtered by the primary filter. Furthermore, we propose Knowledge-Integrated Prediction (KIP), which calibrates the outputs of the adapting model, EMA model, and source model to integrate their complementary knowledge for OSTTA. We validate our approach across diverse closed-set and open-set datasets. Our method enhances both closed-set accuracy and open-set discrimination over existing methods. The code is available at https://github.com/powerpowe/PAF-KIP-OSTTA .

==> sec/2_related.tex <==
\section{Related Works}
\paragraph{Test-Time Adaptation}
Test-time adaptation enables a trained model to adapt to new domains during testing, aiming to mitigate performance degradation when the training and test domains differ \cite{chen2022adacon, sinha2023test, dobler2023rmt, liang2024survey}. This assumes an environment where unlabeled test data is continuously streamed, and the model learns the test domain during inference. Most TTA algorithms are designed to improve the reliability of the model’s predictions \cite{wang2021tent, gong2022note,  niu2022eata}. For instance, Tent \cite{wang2021tent} optimizes the model at test time by minimizing the entropy of the test data. Subsequently, CoTTA \cite{wang2022continual} introduced a practical scenario where domains shift continuously, and many recent TTA studies have adopted CoTTA's domain setting for performance evaluation \cite{gan2023decorate, liu2023vida, gao2024unient}.
\vspace{-1.1cm}
\paragraph{Various Scenarios in Test-Time Adaptation}
TTA research is also advancing by considering more challenging test scenarios. For example, some studies explore environments where the class distribution at test time is non-iid (non-independent and identically distributed) \cite{gong2022note, yuan2023robust, tomar2024mixing}. This causes the model to learn biased knowledge toward certain classes, significantly reducing generalization performance and accumulating errors for other classes. To prevent error accumulation in such environments, they use a strategy like memory buffer \cite{gong2022note} or stable batch normalization \cite{kang2025membn} to prevent error accumulation. 

On the other hand, some recent studies have considered open-set TTA \cite{gao2024unient, lee2023ostta, gong2024sotta, yu2025stamp}. OSTTA \cite{lee2023ostta} avoids training on samples with confidence levels lower than those of the source model. SoTTA \cite{gong2024sotta} and STAMP \cite{yu2025stamp} address error accumulation by placing reliable samples in a memory buffer and repeatedly training on them, thereby preventing errors associated with open-set data. UniEnt \cite{gao2024unient} attempts to learn the distribution of open-set data. UniEnt leverages the knowledge of a fixed source model to evaluate data confidence, clustering data with high and low confidence using a Gaussian Mixture Model. It minimizes entropy for high-confidence data and maximizes entropy for low-confidence data. Nevertheless, UniEnt filters data using a fixed source model, which restricts its ability to effectively leverage domain knowledge and leads to the misidentification of a number of low-confidence closed-set samples as open-set. This paper proposes a filtering approach that prevents error accumulation while considering domain knowledge.


